ResFi: A Secure Framework for Self Organized Radio Resource Management in Residential WiFi Networks

In dense deployments of residential WiFi networks individual users suffer performance degradation due to both contention and interference. While Radio Resource Management (RRM) is known to mitigate this effects its application in residential WiFi networks being by nature unplanned and individually managed creates a big challenge. We propose ResFi - a framework supporting creation of RRM functionality in legacy deployments. The radio interfaces are used for efficient discovery of adjacent APs and as a side-channel to establish a secure communication among the individual Access Point Management Applications within a neighborhood over the wired Internet backbone. We have implemented a prototype of ResFi and studied its performance in our testbed. As a showcase we have implemented various RRM applications among others a distributed channel assignment algorithm using ResFi. ResFi is provided to the community as open source.

==> config.tex <==
%!TEX root = ../techreport.tex

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{graphicx}

\usepackage{tikz}
\usepackage{lipsum}

\usepackage[headsepline,plainheadsepline,footsepline,plainfootsepline]{scrpage2}


\usepackage{mathptmx}
\usepackage[scaled=.92]{helvet}
\usepackage{courier}

% ================================================================
% FIXME package setup
% ================================================================
\usepackage[multiuser,nomargin,marginclue,footnote]{fixme}
% use different colors for fixme levels
\fxusetheme{color}
\fxsetup{targetlayout=colorcb}
% define authors for fixme
% \FXRegisterAuthor{commnad prefix}{environment prefix}{tag}
\FXRegisterAuthor{awo}{anawo}{AWO}
\FXRegisterAuthor{mc}{anmc}{Mikolaj}
% Usage example \mcfatal{Has to be fixed ASAP}
% Usage example \mcerror{Problem}
% Usage example \mcwarning{Possible problem}
% Usage example \mcnote{Comment}
% fixme mode
% change 'draft' to 'final' for final version
\fxsetup{status=draft}


% ================================================================
% Page Style
% ================================================================

\usepackage{geometry}
\geometry{a4paper, inner=30mm, outer=25mm, top=40mm, bottom=42mm}


\clearscrheadfoot

\ihead[\Large {\scshape TU Berlin }]{\Large {\scshape TU Berlin }}

\ifoot[{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}]{{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}}
\cfoot[\scriptsize \trnumber]{\scriptsize \trnumber}
\ofoot[Page \pagemark]{Page \pagemark}

\pagestyle{scrheadings}

\addtokomafont{pagefoot}{\normalfont}



\bibliographystyle{plain}

